DH-GAN: A Physics-driven Untrained Generative Adversarial Network for 3D Microscopic Imaging using Digital Holography

Digital holography is a 3D imaging technique by emitting a laser beam with a plane wavefront to an object and measuring the intensity of the diffracted waveform, called holograms. The object's 3D shape can be obtained by numerical analysis of the captured holograms and recovering the incurred phase. Recently, deep learning (DL) methods have been used for more accurate holographic processing. However, most supervised methods require large datasets to train the model, which is rarely available in most DH applications due to the scarcity of samples or privacy concerns. A few one-shot DL-based recovery methods exist with no reliance on large datasets of paired images. Still, most of these methods often neglect the underlying physics law that governs wave propagation. These methods offer a black-box operation, which is not explainable, generalizable, and transferrable to other samples and applications. In this work, we propose a new DL architecture based on generative adversarial networks that uses a discriminative network for realizing a semantic measure for reconstruction quality while using a generative network as a function approximator to model the inverse of hologram formation. We impose smoothness on the background part of the recovered image using a progressive masking module powered by simulated annealing to enhance the reconstruction quality. The proposed method is one of its kind that exhibits high transferability to similar samples, which facilitates its fast deployment in time-sensitive applications without the need for retraining the network. The results show a considerable improvement to competitor methods in reconstruction quality (about 5 dB PSNR gain) and robustness to noise (about 50% reduction in PSNR vs noise increase rate).

==> discussion.tex <==

Digital holography (DH) has been used to perceive the shallow depth of micro-objects for decades. Compare to the off-axis digital holography, digital in-line holography is much easier to access when advanced optic equipment is not required for this type of setup. 
In the past decades, research groups have tried different methods to solve the in-line holography. For instance, iterative algorithms \cite{latychevskaia2019iterative}, 2D image processing \cite{mcelhinney2009digital}, etc. The achieved results are usually not desirable for this type of problem, which is non-linear and non-inverse. Which decides that this technology will inevitably fade away from people's focus. However, deep neural networks have promised unbelievable achievements in various fields especially in computer vision. Due to the extraordinary performance of complex function approximation and inference, a well-trained neural network reconstructs the phase information from a single-shot hologram is extremely fast. This revolution pushed the application of single-shot in-line digital holograms to a bright side.





An end-to-end network trained with a large dataset usually acquired good performance for image processing tasks. However, for non-inverse problems such as phase reconstruction of single-shot digital holography, a large dataset is difficult to build, or hard to find an existed one that fits the type of current task. Researchers tried to construct artificial datasets for neural networks training \cite{yin2019digital,wang2018eholonet}, and unsurprisingly, they work well [due to their extraordinary performance of the complex function approximating]. However, the trained network may not suitable for a problem that comes from a field where the sample type and imaging parameters are totally different. For instance, an auto-encoder that is trained for the 2D simulated phase reconstruction task may lead to a terrible result when apply it to recover the phase information of nano-cell samples in reality. Through our experiment, the main factor that causes this problem is that the wights of the trained network for a monotonic problem could be totally different from another problem as the training process goes by.  \sout{This type of problem is also known as catastrophic forgetting [].} \xc{This is not called catastrophic forgetting.}

In previous works \cite{li2020deep}, we have developed DeepDIH to retrieve the phase information from simulated holograms. The reconstructed image has purposed promising results compared to the compressive sensing method \cite{zhang2018twin}. When we put the network to recover real holograms captured by the digital camera, the amplitude approaches the expected baseline, however, the reconstructed phase smears and losses a lot of resolution. The reason could be that the embedded auto-encoder network in DeepDIH only has advantages on simulated holograms since its phase and amplitude are highly correlated with each other. Another hypothesis is that the MSE loss function used in the network has a different standard from humans to judge the quality of reconstruction.

Thus, compared to DeepDIH, the DIHGAN delivered results that are much smooth and clear, no matter in broad numerical evaluations or in the actual sensing of bare eyes. More importantly, the proposed GAN architecture in this paper is relatively primary compared to other mature generative-type of networks that are used for super-resolution or denoising. There is still plenty of room for us to improve in future development. For instance, implementing wavelet transform in hologram preprocessing to separate error terms from the principle signals in a prior stage. 

However, a lot of problems have not been solved by the benefits of deep learning in this work. The relocation of object-sensor distance still needs to be calculated in a conventional way. Another problem is that we are hard found a good trade-off point that satisfies both reconstruction quality and time cost, which push the ordinary use of digital holography into a dangerous situation. More importantly, a well-trained network performs surprisingly well in similar reconstruction tasks but achieves catastrophic results for a different types of images. This keeps us confusing: is there a universal solution for all similar non-inverse problems?






==> draft.tex <==
\begin{proof} 

\begin{align}
    \min \mathcal{L}_{TV}&= \min \int_{\Omega} \Bigl| \nabla\angle z\Bigr| \mathbf{d}x\mathbf{d}y \\ \nonumber
    &=  \min\int_{\Omega}\left|\nabla\arctan\frac{\Im(z)}{\Re(z)}\right|\mathbf{d}x\mathbf{d}y\\ \nonumber
    % &= \int_{\Omega}\min \frac{1}{1+(\frac{\Re_x(z)}{\Im_x(z)})^2}+\frac{1}{1+(\frac{\Re_y(z)}{\Im_y(z)})^2} \mathbf{d}x\mathbf{d}y\\ \nonumber
    % \min\sum_{x, y}\left|\angle z_{x+1, y}-\angle\right|_{x, y}+\left|\angle z_{x, y+1}-\angle z_{x, y}\right| \\ \nonumber
    % \\ \nonumber
    % &=\sum_{x, y}\min \left|\left| z\right|_{x+1, y}-\left| z\right|_{x, y}\right| + \min \left|\left| z\right|_{x, y+1}-\left| z\right|_{x, y}\right| \\
\end{align}
% We have,
% \begin{align}
%   \lim_{\Im(z) \to 0}  \frac{\mathbf{d}\frac{1}{1+(\frac{\Im(z)}{\Re(z)})^2}}{\mathbf{d}\Im(z)} = 0
% \end{align}
% and,
% \begin{align}
%   \lim_{\Re(z) \to 0}  \frac{\mathbf{d}\frac{1}{1+(\frac{\Im(z)}{\Re(z)})^2}}{\mathbf{d}\Re(z)} = 0
% \end{align}. Thus, $\lim_{\Im(z) \to 0}$ and $\lim_{\Re(z) \to 0}$ is a local minima of the optimization problem $ \min \mathcal{L}_{TV}$. 
We look one dimension of the signal, and observed,
\begin{align}
   \left|\nabla_x\arctan\frac{\Im(z)}{\Re(z)}\right| =  \left|\frac{1}{1+(\frac{\Im(z)}{\Re(z)})^2}\cdot \frac{\Re(z)\nabla_x \Im(z) -  \Im(z)\nabla_x \Re(z)  }{(\Re(z))^2}\right|
\end{align}
when $\frac{\Im(z)}{\Re(z)}=\frac{\nabla_x \Im(z)}{\nabla_x \Re(z)}$, $ \left|\nabla_x\arctan\frac{\Im(z)}{\Re(z)}\right|$ reaches its minimum. Let $\delta$ denotes $ \left|\nabla_x\arctan\frac{\Im(z)}{\Re(z)}\right|$, to find a minima, we set $\frac{\partial \delta}{\partial \nabla_x \Im(z) } = 0$ and $\frac{\partial \delta}{\partial \nabla_x \Re(z) } = 0$. We have,
\begin{align}
    \frac{\partial \delta}{\partial \nabla_x \Im(z) }  &= -\frac{1}{(1+(\frac{\nabla_x\Im(z)}{\nabla_x\Re(z)})^2)^2}\cdot\frac{2}{(\nabla_x\Re(z))^2}\cdot \nabla_x\Im(z) \\ \nonumber
    \frac{\partial \delta}{\partial \nabla_x \Re(z) }  &= -\frac{1}{(1+(\frac{\nabla_x\Im(z)}{\nabla_x\Re(z)})^2)^2}\cdot (\nabla_x\Im(z))^2\cdot \frac{2}{(\nabla_x\Re(z))^3}
\end{align}
Now, we obtain $\lim_{\left|\nabla_x\Re(z)\right| \to \infty} \frac{\partial \delta}{\partial \nabla_x \Im(z) } =0$ and $\lim_{\left|\nabla_x\Re(z)\right| \to \infty}\frac{\partial \delta}{\partial \nabla_x \Re(z) } =0$. Therefore, when we minimizing the  background loss $\mathcal{L}_{B}$ is the progress to search a local minima of the TV loss operating on the phase.





% \begin{align}
%     \min \mathcal{L}_{TV}&= \min \int_{\Omega} \Bigl| \nabla\left| z\right|~\Bigr| \mathbf{d}x\mathbf{d}y \\ \nonumber
%     &= \min\sum_{x, y}\left|\left| z\right|_{x+1, y}-\left| z\right|_{x, y}\right|+\left|\left| z\right|_{x, y+1}-\left| z\right|_{x, y}\right| \\ \nonumber
%     &=\sum_{x, y}\min \left|\left| z\right|_{x+1, y}-\left| z\right|_{x, y}\right| + \min \left|\left| z\right|_{x, y+1}-\left| z\right|_{x, y}\right| \\
% \end{align}
% Let's look at the term $\left|\left| z\right|_{x+1, y}-\left| z\right|_{x, y}\right|$, which can also be written as 
% \begin{align} \label{eq:term1}
%     \nabla_x\left| z_{x, y}\right| =&\left|\left| z\right|_{x+1, y}-\left| z\right|_{x, y}\right| \\ \nonumber
%     = & \left|\sqrt{\Re^2(z_{x+1, y})+\Im^2(z_{x+1, y})}-\sqrt{\Re^2(z_{x, y})+\Im^2(z_{x, y})}\right|
% \end{align}
% where, $\Re(z_{x+1, y}) = \Re(z_{x, y})+ \nabla_x  \Re(z_{x, y})$ and $\Im(z_{x+1, y}) = \Im(z_{x, y})+ \nabla_x  \Im(z_{x, y})$. Now, Eq. \ref{eq:term1} becomes,
% \begin{align}
%     \nabla_x\left| z_{x, y}\right|& = \Big|\sqrt{\Re^2(z_{x, y})+\Im^2(z_{x, y})  
% + (\nabla_x\Re(z_{x, y}))^2+ (\nabla_x\Im(z_{x, y}))^2+2 \Re(z_{x, y})\nabla_x  \Re(z_{x, y})+2\Im(z_{x, y})\nabla_x  \Im(z_{x, y})}\\ \nonumber
% &+\sqrt{\Re^2(z_{x, y})+\Im^2(z_{x, y})} \Big| \\ \nonumber
% &\leq \sqrt{\left| (\nabla_x\Re(z_{x, y}))^2+ (\nabla_x\Im(z_{x, y}))^2+2 \Re(z_{x, y})\nabla_x  \Re(z_{x, y})+2\Im(z_{x, y})\nabla_x  \Im(z_{x, y}) \right|}
% \end{align}
% \begin{align}
%     |\sqrt{a}-\sqrt{b}|\leq \sqrt{|a-b|},~a>0,~b>0
% \end{align}


\end{proof}
\begin{proof} 

\begin{align}
    \min \mathcal{L}_{TV}&= \min \int_{\Omega} \Bigl| \nabla\angle z\Bigr| \mathbf{d}x\mathbf{d}y \\ \nonumber
    &=  \min\int_{\Omega}\left|\nabla\arctan\frac{\Re(z)}{\Im(z)}\right|\mathbf{d}x\mathbf{d}y\\ \nonumber
    % &= \int_{\Omega}\min \frac{1}{1+(\frac{\Re_x(z)}{\Im_x(z)})^2}+\frac{1}{1+(\frac{\Re_y(z)}{\Im_y(z)})^2} \mathbf{d}x\mathbf{d}y\\ \nonumber
    % \min\sum_{x, y}\left|\angle z_{x+1, y}-\angle\right|_{x, y}+\left|\angle z_{x, y+1}-\angle z_{x, y}\right| \\ \nonumber
    % \\ \nonumber
    % &=\sum_{x, y}\min \left|\left| z\right|_{x+1, y}-\left| z\right|_{x, y}\right| + \min \left|\left| z\right|_{x, y+1}-\left| z\right|_{x, y}\right| \\
\end{align}
% We have,
% \begin{align}
%   \lim_{\Re(z) \to 0}  \frac{\mathbf{d}\frac{1}{1+(\frac{\Re(z)}{\Im(z)})^2}}{\mathbf{d}\Re(z)} = 0
% \end{align}
% and,
% \begin{align}
%   \lim_{\Im(z) \to 0}  \frac{\mathbf{d}\frac{1}{1+(\frac{\Re(z)}{\Im(z)})^2}}{\mathbf{d}\Im(z)} = 0
% \end{align}. Thus, $\lim_{\Re(z) \to 0}$ and $\lim_{\Im(z) \to 0}$ is a local minima of the optimization problem $ \min \mathcal{L}_{TV}$. 
We look one dimension of the signal, and observed,
\begin{align}
   \left|\nabla_x\arctan\frac{\Re(z)}{\Im(z)}\right| =  \left|\frac{1}{1+(\frac{\Re(z)}{\Im(z)})^2}\cdot \frac{\Im(z)\nabla_x \Re(z) -  \Re(z)\nabla_x \Im(z)  }{(\Im(z))^2}\right|
\end{align}
when $\frac{\Re(z)}{\Im(z)}=\frac{\nabla_x \Re(z)}{\nabla_x \Im(z)}$, $ \left|\nabla_x\arctan\frac{\Re(z)}{\Im(z)}\right|$ reaches its minimum. Let $\delta$ denotes $ \left|\nabla_x\arctan\frac{\Re(z)}{\Im(z)}\right|$, to find a minima, we set $\frac{\partial \delta}{\partial \nabla_x \Re(z) } = 0$ and $\frac{\partial \delta}{\partial \nabla_x \Im(z) } = 0$. We have,
\begin{align}
    \frac{\partial \delta}{\partial \nabla_x \Re(z) }  &= -\frac{1}{(1+(\frac{\nabla_x\Re(z)}{\nabla_x\Im(z)})^2)^2}\cdot\frac{2}{(\nabla_x\Im(z))^2}\cdot \nabla_x\Re(z) \\ \nonumber
    \frac{\partial \delta}{\partial \nabla_x \Im(z) }  &= -\frac{1}{(1+(\frac{\nabla_x\Re(z)}{\nabla_x\Im(z)})^2)^2}\cdot (\nabla_x\Re(z))^2\cdot \frac{2}{(\nabla_x\Im(z))^3}
\end{align}
Now, we obtain $\lim_{\left|\nabla_x\Im(z)\right| \to \infty} \frac{\partial \delta}{\partial \nabla_x \Re(z) } =0$ and $\lim_{\left|\nabla_x\Im(z)\right| \to \infty}\frac{\partial \delta}{\partial \nabla_x \Im(z) } =0$. Therefore, when we minimizing the  background loss $\mathcal{L}_{B}$ is the progress to search a local minima of the TV loss operating on the phase.





% \begin{align}
%     \min \mathcal{L}_{TV}&= \min \int_{\Omega} \Bigl| \nabla\left| z\right|~\Bigr| \mathbf{d}x\mathbf{d}y \\ \nonumber
%     &= \min\sum_{x, y}\left|\left| z\right|_{x+1, y}-\left| z\right|_{x, y}\right|+\left|\left| z\right|_{x, y+1}-\left| z\right|_{x, y}\right| \\ \nonumber
%     &=\sum_{x, y}\min \left|\left| z\right|_{x+1, y}-\left| z\right|_{x, y}\right| + \min \left|\left| z\right|_{x, y+1}-\left| z\right|_{x, y}\right| \\
% \end{align}
% Let's look at the term $\left|\left| z\right|_{x+1, y}-\left| z\right|_{x, y}\right|$, which can also be written as 
% \begin{align} \label{eq:term1}
%     \nabla_x\left| z_{x, y}\right| =&\left|\left| z\right|_{x+1, y}-\left| z\right|_{x, y}\right| \\ \nonumber
%     = & \left|\sqrt{\Re^2(z_{x+1, y})+\Im^2(z_{x+1, y})}-\sqrt{\Re^2(z_{x, y})+\Im^2(z_{x, y})}\right|
% \end{align}
% where, $\Re(z_{x+1, y}) = \Re(z_{x, y})+ \nabla_x  \Re(z_{x, y})$ and $\Im(z_{x+1, y}) = \Im(z_{x, y})+ \nabla_x  \Im(z_{x, y})$. Now, Eq. \ref{eq:term1} becomes,
% \begin{align}
%     \nabla_x\left| z_{x, y}\right|& = \Big|\sqrt{\Re^2(z_{x, y})+\Im^2(z_{x, y})  
% + (\nabla_x\Re(z_{x, y}))^2+ (\nabla_x\Im(z_{x, y}))^2+2 \Re(z_{x, y})\nabla_x  \Re(z_{x, y})+2\Im(z_{x, y})\nabla_x  \Im(z_{x, y})}\\ \nonumber
% &+\sqrt{\Re^2(z_{x, y})+\Im^2(z_{x, y})} \Big| \\ \nonumber
% &\leq \sqrt{\left| (\nabla_x\Re(z_{x, y}))^2+ (\nabla_x\Im(z_{x, y}))^2+2 \Re(z_{x, y})\nabla_x  \Re(z_{x, y})+2\Im(z_{x, y})\nabla_x  \Im(z_{x, y}) \right|}
% \end{align}
% \begin{align}
%     |\sqrt{a}-\sqrt{b}|\leq \sqrt{|a-b|},~a>0,~b>0
% \end{align}


\end{proof}

==> excluded_text.tex <==
%Observing the internal structure of micro objects has been a mysterio topic since last century. Dennis Gabor, accidently found a way to explore the distribution of a transparent sample when he was only trying to improve the resolution of the electron microscopes which was just invented at that time. By simply taking away all lenses that are between the samples and the sensor, the electromagnetic wave would pass through the sample directly, forming a specific pattern that includes multi-dimensional information. Gabor indicates that part of the electron wave would interact with the sample and scatter, while another part would pass through without scattering. These two scattered and unscattered waves interact with each other and will propagate an interference pattern which contains the information that indicates both chromatic property and vertical features of the micro objects.

% \arr{check refs for accurate modeling or presentation, in general if we call reference wave as $R(x,y)$ in the object plane, after traveling distance z it should be $R(x,y)e^{-kz}$, unless we define it in the hologram plane.}\xc{Yes, should be in the detector plane}, respectively. The notation $(\cdot)^*$ denotes complex conjugation.


%\arr{Move this to the technical part. up to here is good enough for the introduction}. \fbox{from here}

%\arr{This is a good and easy resource to read: $http://light.ece.illinois.edu/ECE460/PDF/Holography.pdf$ and $https://light.ece.illinois.edu/ECE460/$ in general.}


%Generally, there exist two configurations for DH, including \textit{off-axis} and \textit{in-line} [Garbor] digital holography \cite{gabor1948new}. The twin images $O(x,y)^*R(X,y)$ and $R(x,y)^*O(X,y)$ %reference wave and object wave 
%in the off-axis system are spatially separated, which eliminates the twin image problem.  However, this approach has key restrictive issues of potential information loss by spatial filtering in the Fourier domain, inefficient use of CCD cells, and also requires more complex equipment setup to split and mixing the reference and object waves [XXX]. 
%In contrast, the in-line system is more compact and easier to implement. This system only requires aligning the objective field with a single reference beam, and hence the CCD efficiently samples the formed hologram. However, numerical methods should be used to solve the twin-image problem, since the cross-correlation terms are not spatially separated. A general in-line system is shown in Fig. \ref{fig:in-line}.



%izis the , and $O(x,y)$ is the object wave, (the wave after confronting the object in x-y plane), then the resulting wave is $O(x,y) + R(x,y)$..., }\arr{include accurate formulation here, and mention different terms of the hologram, mention transition function, and forward propagation after traveling distance z, .... Fora clear and accurate definitions, read ref papers, tutorials. I also encourage you to watch educational and lecture videos, like for off-axis you can watch :  $https://www.youtube.com/watch?v=9hgQyx1He_U$, for inline or general DH: $https://www.youtube.com/watch?v=ezyT3gg3YNk$ , $https://www.youtube.com/watch?v=UT4Zt8lgElM$, ....}
%\xc{This part was included in the related work section. I moved it to here.}
% \subsection{Digital Holography and Twin-image problem} \label{sec:twin-image}
%\xc{The added Digital Holography and Twin-image problem below this line}

%The diffraction theory can appropriately characterize the propagation of optical fields, which is friendly for the physics-driven reconstruction approaches
%\ar{put where appropriate}\cite{kim2010principles}. 
%Theoretically, a captured hologram $\mathbf{H}(x,y)$ is presented as:






\arr{not sure but I still believe that $H$ should/can be defined as $H=|O+R|^2$. Review REF papers and bring them with you, or share in a folder, so we can discuss tomorrow.}
\xc{\url{https://www.google.com/books/edition/_/prdEtWNAx64C?hl=en&gbpv=1&pg=PR1&dq=digital+holography+lecture} page 4. and \url{https://opg.optica.org/ao/abstract.cfm?uri=ao-54-9-2424}}  






%\fbox{the rest of this section is technical and can go to the technical sections. Here we just say [one paragraph] to mention our contrast with previous work and our contributions. Like we say we use GAN to realize semantic similarity and model back propagation, then we mention  progressive masking function with simulated annealing and imposing smoothness on the background [we can view it as a hand-tuned visual attention?!!!]. Then we complete the introduction/related work and then elaborate on details in the technical section.}

% This is different from the general GAN. Let's recap the loss of a general GAN \cite{goodfellow2014generative}:
% \begin{equation}
%  \mathcal{L} =\min_G\max_D\mathbb{E}_{x\sim P_{data}}\log[D(x)]+\mathbb{E}_{z\sim p_z}\log[1-D(G(z))],
% \end{equation}  
% where $D(x)$ is the discriminator's estimation of the probability of the real data, $G(z)$ is the generator's output with given input (noise or other) distribution $z\sim p_z$, $D(G(z))$ is the discriminator's estimate of the probability that a fake \arr{here we dont have a fake image rather reproduced one, and we should say the generator is trained so that reproduced holograms are so close to the real ones that fool the discriminator} instance is real. We note here, the discriminator aims to distinguish the difference between distributions of real data and the generated data. The target is to learn the distribution $x\sim P_{data}$ to approximate the real data distribution. When the net only has one fixed input and one fixed output ground truth pair, $ P_{data}$ and $p_z$ become a Dirac delta function $\delta(x)$:
% \begin{align}
%     \delta(x-\xi)= \begin{cases}+\infty, & x=\xi\\ 0, & x \neq \xi\end{cases}
% \end{align}
% It is easy to observed, when optimizing the generator,
% its objective function is presented as,
% \begin{align}\label{eq:gen}
%     &\min_G \log[1-D(G(z))] = \min_G\text{BCE}(G(z),x).    
% \end{align}
% \arr{we can see it in a different view. We don't want to recover the input distribution to call it a delta function, here the generator tries to mimic the nonlinear operation between the hologram and the object wave, ($f_W(H)=|U'|, <U'$, so that $|U'|, <U'$ is as close as possible to ground truth $|U|, <U$, but instead of using MSE and norm2, we use a discriminator network to compare the reproduced versions, or equivalently their forward propagated versions, their corresponding holograms.}





%After optimization, the reconstructed object in complex domain is presented as $\mathbf{O}^* =G^*(z)$.

%The loss is presented in Eq. \ref{eq:loss}, where $\mathbf{H}:\mathbb{R}^{  H \times  W \times 1}$ denotes the captured hologram, and $W$ and $H$ denote the width and the height, respectively. $z:\mathbb{R}^{  H \times  W \times 2}$ denotes the fixed input of the net, and we generally set it as $T_b(\mathbf{H}):\mathbb{R}^{  H \times  W \times 1} \rightarrow\mathbb{R}^{  H \times  W \times 2}$, which is the back-propagation of $\mathbf{H}$ by angular spectrum propagation (ASP).  $G(\cdot):\mathbb{R}^{  H \times  W \times 2} \rightarrow\mathbb{R}^{  H \times  W \times 2}$ and $D(\cdot):\mathbb{R}^{  H \times  W \times 1} \rightarrow\mathbb{R}^{1}$ denote the operators of generator and  discriminator, respectively. $T_f(\cdot):\mathbb{R}^{  H \times  W \times 2} \rightarrow\mathbb{R}^{  H \times  W \times 1}$ denotes the  forward-propagation operator.   $\mathcal{L}_{Auto}$ and $\mathcal{L_{B}}$ denote the autoencoder loss from DeepDIH with its weight $\lambda_1$ and the background loss with its weight $\lambda_2$, respectively. 
% \begin{align}\label{eq:loss}
%     \mathcal{L}=\min _{G} \max _{D} \log [D(\mathbf{H})]+ \log [1-D(T_f(G(z)))]+\lambda_1 \mathcal{L}_{Auto}(G(z))+\lambda_2 \mathcal{L_{B}}(G(z))
% \end{align}
% After optimization, the reconstructed object in complex domain is presented as $\mathbf{O}^* =G^*(z)$.




\subsubsection{Learnable Penalty by GAN structure}\label{sec:gan}
The essential architecture of our work is a self-supervised GAN (shown in Fig \ref{fig:framwork}), which is different from the general GAN. Let's recap the loss of a general GAN \cite{goodfellow2014generative}:
\begin{equation}
 \mathcal{L} =\min_G\max_D\mathbb{E}_{x\sim P_{data}}\log[D(x)]+\mathbb{E}_{z\sim p_z}\log[1-D(G(z))],
\end{equation}  
where $D(x)$ is the discriminator's estimation of the probability of the real data, $G(z)$ is the generator's output with given input (noise or other) distribution $z\sim p_z$, $D(G(z))$ is the discriminator's estimate of the probability that a fake instance is real. 


\fbox{XC: This content below may not be necessary}

If we use  $1$ and  $0$ denote the real label and the fake label, also, according to the binary cross entropy loss, 
\begin{align}
    \mathcal{L}_{BCE}(P_y,P_x)=-\mathbb{E}\left[y_{n} \cdot \log x_{n}+\left(1-y_{n}\right) \cdot \log \left(1-x_{n}\right)\right]
\end{align}
where $P_x$ and $P_y$ are the distributions of the predicted data and the target data, and $y_{n}$ denotes the probability that the target  sample $n$ is $c_0$, which is either 0 or 1, $x_n$ denotes the probability of the predicted data is $c_0$.
 the loss of discriminator $D$ can also be presented as:
  \begin{align}
      \max_D\mathcal{L}_D =& \min -\mathbb{E}_{x\sim P_{data}}\log[D(x)]-\mathbb{E}_{z\sim p_z}\log[1-D(G(z))] \\ \nonumber
       = &\min\mathcal{L}_{BCE}(P_{data},\widetilde{P}_{data})+  \mathcal{L}_{BCE}({P}_{G},\widetilde{P}_{G})
  \end{align}

Similarly, the loss of the generator $G$  can be respectively presented as:
\begin{align}
    \min_G\mathcal{L}_G = \mathbb{E}_{z\sim p_z}\log[1-D(G(z))] \iff&\min-\mathbb{E}_{z\sim p_z}[\log (D(G(z))]\\ \nonumber
                  =& \min\mathcal{L}_{BCE}(P_{data},\widetilde{P}_G)               
\end{align}
\fbox{XC: This content above may not be necessary}

where $P_{data}$ denote the distribution of the real samples, $\widetilde{P}_{data}$ denotes the estimated distribution of the real samples by $D$,  ${P}_{G}$ denotes the distribution of the generated samples, and $\widetilde{P}_{G}$ denotes the estimated distribution of the generated (fake)  samples by $D$. 
In our case, When the net only has one fixed input and one fixed output ground truth pair, $ P_{data}$,  $\widetilde{P}_{data}$, $P_G$, and $\widetilde{P}_{G}$ become a Dirac delta function $\delta(x)$:
\begin{align}
    \delta(x-\xi)= \begin{cases}+\infty, & x=\xi\\ 0, & x \neq \xi\end{cases}
\end{align}
It is easy to observed, when optimizing the generator with well-trained discriminator (meaning $\widetilde{P}_{G}\approx {P}_{G}$),
its objective function is presented as,
\begin{align}\label{eq:gen}
    \min_G -\mathbb{E}_{z\sim p_z}[\log (D(G(z))] &= \mathcal{L}_{BCE}(P_{data},{P}_G)  \\ \nonumber
    &=-p(\mathbf{H})\log p(\hat{\mathbf{H}}=\mathbf{H})
\end{align}
where $p(\mathbf{H})=1$ is fixed, $\hat{\mathbf{H}}$ denotes the reproduced hologram from the net, and the probability $p(\hat{\mathbf{H}}=\mathbf{H})$ is expected to be as large as possible, which indicates that the network is trying to minimize the similarity between $\mathbf{H}$ and $\hat{\mathbf{H}}$.




\arr{don't use the term "fake". just say reproduced hologram or object wave, and we should say the generator is trained so that reproduced holograms are so close to the real ones that fool the discriminator}  

% We note here, the discriminator aims to distinguish the difference between distributions of real data and the generated data. The target is to learn the distribution $x\sim P_{data}$ to approximate the real data distribution.

\arr{we can see it in a different view. We don't want to recover the input distribution to call it a delta function, here the generator tries to mimic the nonlinear operation between the hologram and the object wave, ($f_W(H)=|U'|, <U'$, so that $|U'|, <U'$ is as close as possible to ground truth $|U|, <U$, but instead of using MSE and norm2, we use a discriminator network to compare the reproduced versions, or equivalently their forward propagated versions, their corresponding holograms.}


Therefore, the Eq. \ref{eq:gen} can be used to optimize the generate model solely or ensemble with its original loss function. Moreover, since the discriminator $D$ would extract deep features via its multiple layer convolutional layers, its evaluation of the similarity would be more helpful and meaningful. Thus, the generator would learn a more robust representation from the digital hologram to the real object wave.




\subsubsection{Autoencoder Loss}
The autoencoder loss is defined in Eq. \ref{eq:auto}, which aims minimize the gap between the captured hologram and the forward-propagated reconstructed results. When minimizing the autoencoder Loss,
the generator certainly can search the optimal results by tuning its parameters within the parameter space. 
\begin{align}\label{eq:auto}
 \mathcal{L}_{Auto}(X,H)=\frac{1}{H \times  W }\|H-T_f(X)\|_{2}^{2} 
\end{align}



\fbox{Keep this text for our reference, but we already mentioned our contributions}
\textcolor{gray}{In this paper, our key contributions are roughly characterized as:
\begin{itemize}
    \item Propose a untrained GAN framework (shown in Fig \ref{fig:framwork}) that can reconstruct one-shot digital in-line hologram.
    \item Introduce the background loss that perform the regularization on the background of the sample generated by  K-means segmentation with simulated-annealing optimization.
    \item Show the framework are easily transferable to reconstruct the other hologram with similar pattern. 
\end{itemize}}

